Automated Annotation of Evolving Corpora for Augmenting Longitudinal Network Data: A Framework Integrating Large Language Models and Expert Knowledge

Longitudinal network data are essential for analyzing political, economic, and social systems and processes. In political science, these datasets are often generated through human annotation or supervised machine learning applied to evolving corpora. However, as semantic contexts shift over time, inferring dynamic interaction types on emerging issues among a diverse set of entities poses significant challenges, particularly in maintaining timely and consistent annotations. This paper presents the Expert-Augmented LLM Annotation (EALA) approach, which leverages Large Language Models (LLMs) in combination with historically annotated data and expert-constructed codebooks to extrapolate and extend datasets into future periods. We evaluate the performance and reliability of EALA using a dataset of climate negotiations. Our findings demonstrate that EALA effectively predicts nuanced interactions between negotiation parties and captures the evolution of topics over time. At the same time, we identify several limitations inherent to LLM-based annotation, highlighting areas for further improvement. Given the wide availability of codebooks and annotated datasets, EALA holds substantial promise for advancing research in political science and beyond.

==> tables/topics.tex <==
\begin{center}
\begin{longtable}{p{2cm}p{4cm}p{6cm}}
    \caption{Topics Detected by EALA }
    \label{eala_topics}
    \toprule
\multicolumn{1}{c}{Name}	&	\multicolumn{1}{c}{Definition}	&	\multicolumn{1}{c}{Original Topic Words}		\\
\midrule
REDD	&	Topics related to Reducing Emissions from Deforestation and Forest Degradation and its frameworks.	&	redd, qelros, redd+		\\
Governance	&	A focus on administration, accountability, and leadership in the pursuit of climate goals and public engagement.	&	reporting, ambition, historical responsibility, namas, governance, support, targets, public awareness, accountability, awareness, agenda, leadership, administrative matters, poverty eradication, inclusiveness, administration		\\
Stakeholder Engagement	&	Involvement and participation of various stakeholders, including the private sector and LDCs, in climate initiatives.	&	institutional arrangements, ldcs, private sector involvement, public-private partnerships, private sector engagement, private sector, stakeholders, stakeholder involvement, stakeholder participation		\\
Emissions	&	Discussion on emission reduction targets and trading, tackling greenhouse gases and protecting the ozone layer.	&	emission reductions, emissions trading, emissions reduction, emissions, emission reduction, greenhouse gases, emission reduction targets, emission targets, emissions targets, ghg emissions, greenhouse gas emissions, emissions reductions, greenhouse gas inventories, emissions projections, air pollution, ozone layer protection		\\
Climate Science	&	Broad discussions encompassing climate change science, policy, justice, and actions under international agreements.	&	research / climate science, kyoto protocol, climate change, climate science, climate change impacts, climate action, climate policy, climate justice, climate change mitigation, climate variability, extreme weather events, climate modeling, climate change conference		\\
Adaptation Planning	&	Strategies that include just transition, training initiatives, and the development of national adaptation plans with guidance and facilitation support.	&	adaptation, just transition, training, adaptation planning, facilitation, national adaptation plans, guidance, planning		\\
Sustainability	&	Encompassing sustainable development, environmental resilience, and conservation efforts.	&	sustainable development, environmental integrity, biodiversity, environment, sinks, resilience, economic resilience, water resources, sustainability, ecosystems, water, conservation, desertification, ecosystem approach		\\
Assessment	&	Processes of review, evaluation, and verification in climate agendas.	&	review, analysis and assessment, scientific assessments, assessment, evaluation, verification, accreditation		\\
Global Agreements	&	Negotiation and content of international agreements under the UNFCCC framework, including the Paris Agreement, Cancun Agreements, and Marrakesh Accords.	&	content of new agreement, unfccc, paris agreement, agreement, additionality, new agreement, global agreement, cancun agreements, marrakesh accords		\\
Finance	&	Funding and financial arrangements for capacity building, equity, and adaptation impacts.	&	finance, capacity building, equity, budget, adaptation fund, funding, investment, financing, impacts, programme budget, poverty reduction, economic impacts, socioeconomic impacts, supplementarity, economic growth, incentives		\\
Protocols	&	Details on international protocols such as the Montreal Protocol, including ratification processes.	&	protocol, joint implementation, ratification, protocol amendment, protocol ratification, montreal protocol		\\
Data Management	&	Focus on data collection, management, and observations related to climate discussions.	&	data and observations, data collection, data, data management		\\
Mitigation Policies	&	Policies and measures for mitigation, taking into account political will and common but differentiated responsibilities.	&	mitigation, policies and measures, insurance, policies, policy, bali action plan, policy approaches, common but differentiated responsibilities, political will, policy measures, policy and measures		\\
International Cooperation	&	Commitment to global cooperation, shared actions, and long-term partnerships.	&	commitment, international cooperation, action, cooperation, shared vision, participation, coordination, long-term cooperation, long-term cooperative action, workshops, synergies, collaboration, multilateralism, co-benefits, activities implemented jointly, workshop, global cooperation, voluntary commitments		\\
Market Mechanisms	&	Use of market-based mechanisms for economic diversification and financial opportunities.	&	global stocktake, economic diversification, market mechanisms, financial mechanism, market-based mechanisms, markets, market-based opportunities		\\
Compliance	&	Mechanisms and systems for ensuring and addressing compliance and non-compliance in international climate agreements.	&	compliance, compliance system, enforcement, compliance mechanism, compliance mechanisms, non-compliance		\\
Transport	&	Concerns and strategies associated with international transport emissions.	&	international transport, transport		\\
Forestry and Agriculture	&	Management of forests and agriculture, focusing on sustainable practices and indigenous knowledge.	&	agriculture, forests, afforestation and reforestation, deforestation, forestry, forest management, indigenous knowledge, afforestation, sustainable forest management, cross-cutting issues, reforestation		\\
Implementation Methodologies	&	Methodologies and tools for implementing climate initiatives, integrating traditional knowledge.	&	principles, implementation, clean development mechanism, methodological issues, methodologies, methodology, sectoral approaches, means of implementation, guidelines, methods and tools, best practices, traditional knowledge, framework, scientific findings, procedures, modeling, definitions, comparability of efforts		\\
Carbon Management	&	Approaches to carbon capture, storage, and market mechanisms for low-carbon development.	&	carbon capture and storage, carbon market, carbon markets, low-carbon development, carbon sinks, carbon sequestration, carbon neutrality		\\
Organizational Matters	&	Administrative and organizational matters, covering gender balance, employment, decision-making processes, and work programs related to health and international trade.	&	organization, organisation, lulucf, health, work programme, gender, accounting, programme of work, gender equality, business, employment, decision-making, tourism, base year, international trade, gender balance		\\
Energy Transition	&	Emphasis on energy efficiency and renewable sources, alongside nuclear energy as a low-carbon energy option.	&	energy, renewable energy, energy efficiency, nuclear energy		\\
Technology Transfer	&	Facilitating the development and transfer of technology and innovative solutions.	&	technology, transparency, technology transfer, research, education, development, innovation, progress, process, least developed countries, science, tools, resources, uncertainty, technology development and transfer		\\
Negotiation Processes	&	Processes of international negotiations and dialogue for climate commitments.	&	commitments, negotiations, negotiation, negotiation process, trade, compensation, dispute settlement, dialogue		\\
Response Measures	&	Monitoring and metrics for assessing climate response measures and indicators.	&	response measures, monitoring, comparability, indicators, common metrics, measures, ghg inventories, baselines, metrics		\\
Loss and Damage	&	Addressing vulnerability, risk management, disaster risk reduction, early warning systems, safeguards, food security, and disaster management related to climate impacts.	&	loss and damage, vulnerability, adverse effects, disaster risk reduction, food security, risk management, vulnerability assessment, risk assessment, risk reduction, vulnerability assessments, early warning systems, safeguards, vulnerabilities, disaster management		\\
Differentiation and Integration	&	Considerations of differentiation and integration in climate negotiations.	&	differentiation, integration		\\
Human Rights	&	Incorporating human and indigenous rights into climate legal frameworks, considering national circumstances and relevant legal issues.	&	human rights, indigenous peoples, national circumstances, legal issues, legal framework, indigenous rights, amendment, intellectual property rights, legal matters, legal form, amendments, legal options, privileges and immunities		\\
Information Sharing	&	Emphasis on communication and exchange of socio-economic information.	&	national communications, communication, socioeconomic information, information sharing, knowledge sharing, information exchange, contact information, information		\\
Flexibility Mechanisms	&	Inclusion of flexibility in mechanisms for achieving climate-related targets.	&	flexibility mechanisms, flexibility, mechanisms, flexible mechanisms		\\
Talanoa Dialogue	&	A process of inclusive and participatory dialogue to enhance climate action through transparent and constructive discussions.	&	talanoa dialogue		\\
Non-Market Approaches	&	Exploration of alternative approaches to climate actions that exclude market-based mechanisms, focusing on collaboration and capacity-building.	&	non-market approaches, non-market-based approaches		\\
National Adaptation Plans	&	Development and implementation of National Adaptation Plans (NAPs) to systematically address climate resilience and adaptation priorities.	&	naps		\\
Common Time Frames	&	Harmonization and synchronization of time frames for climate action commitments across countries to enhance global comparability, transparency, and accountability.	&	common time frames		\\
Net Zero	&	The ambition to achieve a balance between greenhouse gas emissions produced and those removed from the atmosphere, aiming for climate neutrality.	&	net zero		\\
Decarbonization	&	Efforts and strategies to reduce carbon emissions across various sectors by transitioning to clean and sustainable energy sources, enhancing energy efficiency, and implementing low-carbon technologies and policies.	&	decarbonization		\\
\bottomrule
\end{longtable}
\end{center}
